Generalized Zariski-van Kampen theorem and its application to Grassmannian dual varieties

We formulate and prove a generalization of Zariski-van Kampen theorem on the topological fundamental groups of smooth complex algebraic varieties. As an application, we prove a hyperplane section theorem of Lefschetz-Zariski-van Kampen type for the fundamental groups of the complements to the Grassmannian dual varieties.

==> figADT.tex <==
% figADT.mtask
\renewcommand{\PStextplot}[3]{\rlap{\hskip -108.000000 pt \hbox{\hskip #1pt  \raise #2pt \hbox{#3}}}}%
\begin{figure}
 \begin{center}
 \includegraphics{figADTps.ps}%
\end{center}
\caption{$\varphi\inv (\Sigma\spsh_i)\subset A$ in Corollary~\ref{cor:A}}%
\label{figADT}%
\end{figure}%
